On Event Individuation for Document-Level Information Extraction

As information extraction (IE) systems have grown more adept at processing whole documents, the classic task of template filling has seen renewed interest as benchmark for document-level IE. In this position paper, we call into question the suitability of template filling for this purpose. We argue that the task demands definitive answers to thorny questions of event individuation -- the problem of distinguishing distinct events -- about which even human experts disagree. Through an annotation study and error analysis, we show that this raises concerns about the usefulness of template filling metrics, the quality of datasets for the task, and the ability of models to learn it. Finally, we consider possible solutions.

==> sections/experiments.tex <==
Our primary motivation for using subevents in this work is to reduce the difficulty of individuating events. The IAA results from \S\ref{sec:decomposition} hint that it may help achieve this for humans, but we would like to know whether the same is true for models. In \S\ref{subsec:event_vs_subevent_id}, we evaluate the difficulty of identifying subevents relative to the difficulty of identifying the broader events they constitute, as given by the MUC-4 templates. Then, in \S\ref{subsec:events_from_subevents}, we consider the extent to which events may be identified on the basis of subevents alone.

\subsection{Individuation with OpenAI Models}\label{subsec:event_vs_subevent_id}
In this first set of experiments, we compare the zero-shot performance of ChatGPT (\texttt{gpt-3.5-turbo}) and GPT-4 on template identification vs. subevent identification on the set of reannotated MUC-4 documents. For template identification, we provide a set of instructions in the system prompt that specify criteria for what kinds of events count as valid MUC templates, along with a directive to count the number of distinct incidents of the input type and to provide a justification for its answer (see \autoref{app:openai_experiments} for complete prompt descriptions). For the user prompt, we provide a query of the form \emph{Document: $\langle$text$\rangle$ Event Counts:}. Given the known variability in performance across prompts, we report the modal response across three system prompt variants for each document and input template type.\footnote{For multiple (i.e.\ 3) modes, we break ties in favor of the correct count if possible, and select the smallest count otherwise.}

For subevent identification, we supply a similar set of instructions in the system prompt. In the user prompt, we include the full document text as above, along with a JSON-formatted representation of the subevent decomposition for the template type of interest, ending with the same ``Event counts:'' cue:
\begin{minted}[bgcolor=codebg,mathescape,fontsize=\footnotesize]{js}
{
  "event": "bombing",
  "before": [
    {
      "name": "Motivation",
      "order": 0,
      "description": "<subevent definition>",
      "roles": {
        "Motive": {
          "definition": "<role definition>"
        }, // ...
      }
    }, // ...
  ],
  "during": // ... ,
  "after": // ...
}
\end{minted}

We present the results of these experiments in \autoref{tab:openai_individuation}. Uniformly higher metrics (count accuracy, mean absolute error, and Krippendorff's $\alpha$) for both models on subevent identification suggest that it is an easier task than template identification, echoing the higher IAA among the authors on the former.

\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|ccc}
    \toprule
        Task & Model & $\alpha$ & EM (\%) & MAE \\
    \midrule
        \multirow{4}{*}{Template ID} & Majority (G) & -0.22 & 55.6 & 1.00 \\
        & Majority (T) & \phantom{-}0.22 & 51.1 & 0.89 \\
        & ChatGPT & \phantom{-}0.32 & 57.8 & \textbf{0.78} \\
        & GPT-4 & \phantom{-}\textbf{0.59} & \textbf{62.2} & 0.84 \\
        \midrule
        \multirow{4}{*}{Subevent ID} & Majority (G) & -0.14 & 74.8 & 0.37 \\
        & Majority (T) & \phantom{-}\textbf{0.57} & \textbf{80.9} & \textbf{0.30} \\
        & ChatGPT & \phantom{-}\textbf{0.57} & 78.6 & 0.35 \\
        & GPT-4 & \phantom{-}0.50 & 73.1 & 0.33 \\
    \bottomrule
    \end{tabular}}
    \caption{Performance of (1) Majority (G) (predicts the majority count over all documents); (2) Majority (T) (predicts the majority count by (sub)event type); (3) ChatGPT (\texttt{gpt-3.5-turbo-16k}); and (4) GPT-4 on event and subevent ID on the subset of MUC-4 documents from \S\ref{sec:evaluation}, as measured by (1) (Ratio) Krippendorff's $\alpha$ with the gold counts; (2) exact match accuracy; (3) mean absolute error. Subevent ID performance is higher for both ChatGPT and GPT-4 across all metrics. Best results within task are bolded.}
    \label{tab:openai_individuation}
\end{table}

\subsection{Predicting Events from Subevents}\label{subsec:events_from_subevents}
Subevent identification is clearly valuable insofar as one cares about the fine-grained information it provides. But supposing one's ultimate interests are in broader events, a natural question to ask is how effectively these events can be identified given knowledge of a document's subevent structure. We consider this question now, once again focusing on the zero-shot setting with the same three models from \S\ref{subsec:event_vs_subevent_id}. Thus, the template ID scores in \autoref{tab:openai_individuation} provide a baseline in this setting that leverages no subevent information at all, using only the document as context for the query about event counts. We consider three further settings for evaluation:
\begin{enumerate}
    \item Document + gold subevent annotations
    \item Gold subevent annotations only (no document)
    \item Predicting events counts based on the number of \emph{key} subevents (defined below)
\end{enumerate}
We define the \emph{key} subevent of a decomposition to be the one most canonically associated with the broader event (e.g.\ the \texttt{ignition} subevent for an act of arson or the \texttt{activation} subevent for a bombing; see \autoref{tab:subevent_decomp} for a complete list). This is an admittedly subjective notion, but at least for these decompositions, we think our choices are uncontroversial.

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|ccc}
    \toprule
    Model & Doc. & Sub. & $\alpha$ & Acc (\%) & MAE \\
    \midrule
    Key & N/A & N/A & 0.81 & 73.8 & 0.33 \\
    \midrule
    & $+$ & $-$ & 0.32 & 57.8 & 0.78 \\
    ChatGPT & $-$ & $+$ & 0.12 & 60.0 & 0.87 \\
    & $+$ & $+$ & \textbf{0.37} & \textbf{66.7} & \textbf{0.60} \\
    \midrule
    & $+$ & $-$ & 0.59 & 62.2 & 0.84 \\
    GPT-4 & $-$ & $+$ & 0.62 & 68.9 & \textbf{0.38} \\
    & $+$ & $+$ & \textbf{0.67} & \textbf{75.6} & 0.44 \\
    \bottomrule
\end{tabular}}
\caption{Zero-shot template ID results for different models and settings. $+$/$-$Doc indicates whether or not the document is included in the prompt. $+/-$Sub indicates whether or not gold subevent annotations are included in the prompt. The ``$+$Doc/$-$Sub'' results are the same template ID results from \autoref{tab:openai_individuation}. The ``Key'' baseline predicts events based on key subevent counts (see \S\ref{sec:subevent_experiments}). All ChatGPT and GPT-4 results reflect the modal response across three prompts.}
\label{tab:events_from_subevents}
\end{table}
